Two Transiting Low Density Sub-Saturns from K2

We report the discovery and confirmation of two sub-Saturn planets orbiting a bright (V = 11.3), metal-rich ([Fe/H] = 0.42 $\pm$ 0.04 dex) G3 dwarf in the K2 Campaign 2 field. The planets are 5.68 $\pm$ 0.56 Earth-radii and 7.82 $\pm$ 0.72 Earth-radii and have orbital periods of 20.8851 $\pm$ 0.0003 d and 42.3633$\pm$0.0006 d, near to the 2:1 mean-motion resonance. We obtained 32 radial velocities (RVs) with Keck/HIRES and detected the reflex motion due to EPIC-203771098b and c. These planets have masses of 21.0 $\pm$ 5.4 Earth-masses and 27.0 $\pm$ 6.9 Earth-masses, respectively. With low densities of 0.63 $\pm$ 0.25 g/cc and 0.31 $\pm$ 0.12 g/cc, respectively, the planets require thick envelopes of H/He to explain their large sizes and low masses. Interior structure models predict that the planets have fairly massive cores of 17.6 $\pm$ 4.3 Earth-masses and 16.1 $\pm$ 4.2 Earth-masses, respectively. They may have formed exterior to their present locations, accreted their H/He envelopes at large orbital distances, and migrated in as a resonant pair. The proximity to resonance, large transit depths, and host star brightness offer rich opportunities for TTV follow-up. Finally, the low surface gravities of the EPIC-203771098 planets make them favorable targets for transmission spectroscopy by HST, Spitzer, and JWST.

==> tab_planet-parameters.tex <==
{\renewcommand{\arraystretch}{1.5}
\begin{deluxetable*}{l l l l l}[bt]
\tabletypesize{\scriptsize}
\tablecaption{  Planet Parameters \label{tab:planet}}
\tablewidth{0pt}
\tablehead{
\colhead{Parameter} & \colhead{Units} & \colhead{b} & \colhead{c} 
}
\startdata
\multicolumn{3}{l}{\hspace{1cm} Light curve fitting } \\
   $T_{0}$ & BJD$_\mathrm{TDB} - 2454833$ & $2072.7957\pm0.0010$ &$2082.6247\pm0.0006$ \\
       $P$ &          d & $20.8851\pm0.0005$ &$42.3638\pm0.0008$ \\
       $i$ &        deg & $89.11_{ -0.78 }^{ +0.54 }$ &$89.57_{ -0.24 }^{ +0.28 }$ \\
 $R_P/R_*$ &         \% & $4.39_{ -0.09 }^{ +0.21 }$ &$6.05_{ -0.10 }^{ +0.14 }$ \\
  $T_{14}$ &         hr & $5.42_{ -0.06 }^{ +0.13 }$ &$6.43_{ -0.08 }^{ +0.10 }$ \\
  $T_{23}$ &         hr & $4.87_{ -0.19 }^{ +0.07 }$ &$5.58_{ -0.12 }^{ +0.08 }$ \\
   $R_*/a$ &         -- & $0.036_{ -0.003 }^{ +0.007 }$ &$0.020_{ -0.001 }^{ +0.002 }$ \\
       $b$ &         -- & $0.43_{ -0.25 }^{ +0.24 }$ &$0.37_{ -0.24 }^{ +0.16 }$ \\
       $u$ &         -- & $0.55\pm0.04$ &$0.56\pm0.03$ \\
\rhostarcirc &     \gcc & $0.95_{ -0.41 }^{ +0.26 }$ &$1.31_{ -0.31 }^{ +0.27 }$ \\
\multicolumn{3}{l}{\hspace{1cm} RV fitting } \\
       $K$    & \ms     & $5.1\pm1.2$ &$5.3\pm1.1$ \\
     \ecosw   & --      & $0.20\pm0.09$ &$0.00\pm0.09$ \\   
     \esinw   & --      & $-0.06\pm0.16$ &$-0.02\pm0.15$ \\   
     $e$      & --      & $0.24_{-0.11}^{+0.11}$ & < 0.39 (95\%) \\   
     $\gamma$ & \ms     & \multicolumn{2}{c}{ $-2.7 \pm 1.0$  } \\
     \dvdt    & \msyr   & \multicolumn{2}{c}{ $-22.5 \pm 9.2$  } \\
    \sigjit   & \ms     & \multicolumn{2}{c}{ $2.9 \pm 0.6$  } \\
\multicolumn{3}{l}{\hspace{1cm} Derived Properties } \\
       $a$ &         AU & $0.154\pm0.002$ &$0.247\pm0.004$  \\
     \Sinc &        \Se & $60\pm14$ &$23\pm5$ \\
      \teq &          K & $767\pm177$ &$606\pm139$ \\
       \Rp &        \Re & $5.78\pm0.60$ &$7.97\pm0.75$ \\
       \Mp &        \Me & $23.2\pm5.3$ &$31.0\pm6.4$ \\ 
    $\rho$ & g cm$^{-3}$ & $0.66\pm0.25$ &$0.34\pm0.12$ 
\enddata
\end{deluxetable*}
}

